Exploring space efficiency in a tree-based linear model for extreme multi-label classification

Extreme multi-label classification (XMC) aims to identify relevant subsets from numerous labels. Among the various approaches for XMC, tree-based linear models are effective due to their superior efficiency and simplicity. However, the space complexity of tree-based methods is not well-studied. Many past works assume that storing the model is not affordable and apply techniques such as pruning to save space, which may lead to performance loss. In this work, we conduct both theoretical and empirical analyses on the space to store a tree model under the assumption of sparse data, a condition frequently met in text data. We found that, some features may be unused when training binary classifiers in a tree method, resulting in zero values in the weight vectors. Hence, storing only non-zero elements can greatly save space. Our experimental results indicate that tree models can achieve up to a 95% reduction in storage space compared to the standard one-vs-rest method for multi-label text classification. Our research provides a simple procedure to estimate the size of a tree model before training any classifier in the tree nodes. Then, if the model size is already acceptable, this approach can help avoid modifying the model through weight pruning or other techniques.

==> Makefile <==
# FILES = $(addsuffix .pdf, $(basename $(wildcard *.tex)))
FILES = multilabel_tree_model_size.pdf # to be discussed

all:	$(FILES)

LATEX ?= latex
PDFLATEX ?= pdflatex
BIBTEX ?= bibtex

# rules

TEX_DEPS = *.tex *.sty *.bib

CLEAN_FILES += *.log *.aux *.out *.ilg *.ind *.lof *.lot *.toc \
		*.bbl *.blg \
		*.dvi *.ps *.pdf \
		*.nav *.snm *.vrb *.synctex.gz

.SUFFIXES: .tex .dvi .ps .pdf

.tex.pdf:
	pdflatex --shell-escape $<
	-bibtex $*
	pdflatex --shell-escape $<
	pdflatex --shell-escape $<
	pdflatex --shell-escape $<

clean:
	rm -f $(CLEAN_FILES)


==> section-tree-model-size.tex <==
\section{Inherent Pruning in Tree-based Methods for Sparse Data}
\label{sec:inherent-pruning}
In this section, we explain that for sparse data, the number of weight values needed to be stored in a tree model can be much less than not only the huge value in \eqref{eq:space-for-tree}, but also $nL$, the number of weight values in an OVR model.
We stress that the model size reduction here is not achieved by applying any techniques. 
Instead, it can be regarded as an innate advantage of tree-based methods and we call such reduction ``inherent pruning''.

In the tree-based method, suppose we are training weight vectors at a tree node $u$.
Only a subset of all training instances (specifically, instances having any label in the label subset of $u$) are used.
Because the feature vectors are sparse, some features may have no values in the subset of training instances.
We can remove the unused features before training a multi-label model for the node.
Alternatively, if our optimization algorithm for each binary classification problem \eqref{eq:binary-relevance-loss} satisfies that
\begin{itemize}
  \item the initial $\bw$ is zero, and
  \item for unused features (i.e., feature value are zero across all instances), the corresponding $\bw$ components are never updated, 
\end{itemize}
then we can conveniently feed the subset of data into the optimization algorithm and get a $\bw$ vector with many zero elements.
This way, we keep all weight vectors in all nodes to have the same dimension $n$.
We can collect them as a large sparse matrix for easy use.

We use the name ``inherent pruning'' because the tree-based method itself ``prunes'' weight values for unused features by not updating the corresponding weight components during training.
Our survey shows that few works, except \citep{KJK20a}, mentioned the identity.
Even though, in \cite{KJK20a} the authors only briefly said that ``the weight sparsity increases with the depth of a tree ... implies a significant reduction of space'' without further discussion or experiments.
% The limited coverage of space analysis of tree methods shows that our study is necessary.

% During the training process, dropping these useless features doesn't affect the learned weights since the corresponding components in the weights would be merely zero.
% For the remaining components we still expect nonzero weights as discussed in section \ref{subsec:one-vs-rest}.
% Therefore, it may take less than $n$ (the number of original features) numbers to store a trained weight.
% This explains why it is possible that a tree model needs less space than an OVR model.

\subsection{Case Study}
\label{sec:case-study}
Now we theoretically analyze the size of tree models for sparse data with different tree depths.
Our analysis follows the balanced-tree structure in Figure~\ref{fig:K-ary-tree}.
We choose the OVR model with $Ln$ weight numbers as the comparison baseline because an OVR model is more space-efficiency than a tree model with dense weight matrix, which takes a space of $\hat{L}n$ weight values in \eqref{eq:space-for-tree}.

\begin{table}[t]
  \begin{center}
    \begin{adjustbox}{max width=0.49\textwidth,center}
    \begin{tabular}{c c c c} 
     Depth & \# nodes &\# children / node & \# features \\
     \hline
     0 & $K^0$ & $K$ & $n$ \\ 
     \hline
     1 & $K^{1}$ & $K$ & $\alpha n$ \\
     \hline
     2 & $K^{2}$ & $K$ & $\alpha^2 n$ \\
     \hline
     \vdots & \vdots & \vdots & \vdots\\
     \hline
     $i$ & $K^{i}$ & $K$ & $\alpha^{i} n$\\
     \hline
     \vdots & \vdots & \vdots & \vdots\\
     \hline
     $d-1$ & $K^{d-1}$ & $L/K^{d-1}$ & $\alpha^{d-1} n$
    \end{tabular}
    \end{adjustbox}
  \end{center}
  \caption{\label{tbl:information-of-K-ary-tree} Depth-wise summary of a tree model.}
\end{table}  
\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{fig/fixed-K-with-different-alpha.png}
  \caption{\label{fig:fixed-K-with-different-alpha}The ratio of number of non-zeros between a tree model and an OVR model, calculated based on \eqref{eq:model-size-ratio}. We show the cases for $\alpha=\{0.3, 0.4, 0.5\}$.}
\end{figure}

As the tree depth grows, the training subset becomes smaller and the number of used features also reduces.
Therefore, we assume that when the number of labels is divided by $K$, the number of remaining features is multiplied by a ratio $\alpha \in (0, 1)$.
Based on the assumption, we list the information for each depth in Table~\ref{tbl:information-of-K-ary-tree}.
According to Table~\ref{tbl:information-of-K-ary-tree}, the number of non-zeros to be stored in a tree model is
\begin{align}
  \phantom{=}&\sum_{i=0}^{d-2} (K^{i})(K)(\alpha^{i} n) \nonumber\\
  & \ \ \ \ \ \ + (K^{d-1})\left(\dfrac{L}{K^{d-1}}\right) (\alpha^{d-1}n)\nonumber\\
  \label{eq:tree-model-size}
  &= Kn \cdot \dfrac{(K\alpha)^{d-1}-1}{K\alpha -1} + L\alpha^{d-1}n,
\end{align}
and the ratio of the number of non-zeros in a tree model over an OVR model is
\begin{equation}
  \label{eq:model-size-ratio}
  \dfrac{\text{\eqref{eq:tree-model-size}}}{Ln}
  = \dfrac{K((K\alpha)^{d-1}-1)}{L(K\alpha -1)}+\alpha^{d-1}.
\end{equation}
Usually we choose $K$ to be at least 10, and assume the value for $K\alpha$ is much larger than one.
The reason is that the used features among the label representations must overlap, making a feature still used in more than one of the clusters.
Therefore, we approximate \eqref{eq:model-size-ratio} by 
\begin{align}
    \dfrac{K(K\alpha)^{d-1}}{L(K\alpha)}+\alpha^{d-1}
    &= \alpha^{d-2} \left(\dfrac{K^{d-1}}{L} + \alpha\right)\nonumber\\
    &\le \label{eq:upper-bound} \alpha^{d-2} \left( \dfrac{1}{2} + \alpha \right),
\end{align}
where the last inequality follows from $L \ge 2K^{d-1}$ (the minimum number of labels required to reach depth-$d$ for a balanced tree).
When $\alpha$ is not too close to one, we can expect the upper bound \eqref{eq:upper-bound} smaller than one.
Therefore, for sparse data, the model size in \eqref{eq:tree-model-size} should be smaller than OVR.
Moreover, a deeper tree leads to a smaller model.
We empirically plot the ratio \eqref{eq:model-size-ratio} with $L = 3,000,000$, $K=100$ and different $\alpha$'s in Figure~\ref{fig:fixed-K-with-different-alpha}.
Similar to the derivation, as the tree grows deep, the overall model size reduces, regardless the value of $\alpha$.
Later in Section~\ref{subsec:results-and-discussion}, we shall see that the experiments on real-world data align with our analysis.
